Attention-based hybrid solvers for linear equations that are geometry aware

We present a novel architecture for learning geometry-aware preconditioners for linear partial differential equations (PDEs). We show that a deep operator network (Deeponet) can be trained on a simple geometry and remain a robust preconditioner for problems defined by different geometries without further fine-tuning or additional data mining. We demonstrate our method for the Helmholtz equation, which is used to solve problems in electromagnetics and acoustics; the Helmholtz equation is not positive definite, and with absorbing boundary conditions, it is not symmetric.

==> names.tex <==

\title[Geometry aware hybrid solver]{Geometry aware hybrid solvers for linear equations
}

\author {I. Versano}

\address {School of Mathematical Sciences, Tel-Aviv University, Tel-Aviv 6997801, Israel}

\email {idanversano@tauex.tau.ac.il}

\author {E. Turkel}

\address {School of Mathematical Sciences, Tel-Aviv University, Tel-Aviv 6997801, Israel}

\email {turkel@tauex.tau.ac.il}

%


==> section1.tex <==
	\section{one dimensional results}

\begin{table}[htb!]
	\centering
	\begin{tabular}{|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|}
		\hline
		$N$&k& optimal $J$ &conv. rate&error& iterations	\\ [0.5ex]
		\hline
		$30$&25& 6& 0.15&1e-14&209 \\[1mm]
		$60$&25& 13& 0.04&5e-14&644 \\[1mm]
		$120$&25& 30& 0.01&3.12e-13&2479 \\[1mm]
		$240$&25& 50& 0.002&1.5e-12&9068\\[1mm]
		\hline
		\hline
		
		$30$&35& 5& 0.13&3e-14&233\\[1mm]
		$60$&35& 8& 0.04&6e-14&651 \\[1mm]
		$120$&35& 20& 0.012&3e-13&2299 \\[1mm]
		$240$&35& 12& 0.003&1e-12&8360\\[1mm]
		\hline
	\end{tabular}
	\caption{Hints-GS for 1D-Helmholtz \eqref{eq:helm} with $k=35$ and $f=\sin(\pi x)+10\sin(3\pi x)+10\sin(5\pi x)$.}
	\label{tab:tab1}
\end{table}
We begin by demonstrating our observations on the one-dimensional Helmholtz equation \eqref{eq:helm}
in $(0,1)$
with $k\in \{25,35,50\}$
and Dirichlet boundary conditions. In all our examples, the corresponding linear system admits negative eigenvalues, and so Jacobi, Gauss-Seidel, and Multi-grid do not converge.
The network is trained on data defined over a uniform grid with $N=30$ points. We generate the data points by taking 300 Gaussian random fields $\{f_n\}_{n=1}^{300}$ with zero mean and standard deviation  $0.02$. 
Then, we approximate the corresponding solution for the (discretized) Helmholtz equation to obtain the corresponding $u_n$.

We emphasize that although the network is trained on $N\!=\!30$, we can still use it for inference on other discretizations (see the following subsection) using a pre-interpolation procedure. Hence, the network can be used to solve the equation on higher resolutions than the one used for training.

We point out the following observations:
\begin{itemize}
	
	\item Figure \ref{fig:fig1} (A) demonstrates that $\N$ does not provide by itself a good estimate for the numerical solution
	of Helmholtz equations with $k=50$ and 
	$f=\sin(2\pi x)$ whereas it provides a better approximation for Gaussian random field (right), even when the resolution is the same as the one used for training
	\\[1mm]
	\item Figure \ref{fig:fig1} (B) shows how the behavior of the error along iterations. This behavior is very similar to that pointed out in \cite{zhang}, showing that Deeponet decreases low modes of the error and Gauss-Seidel iterations increase them. The opposite occurs for the higher modes. 
	\\[1mm]
	\item Table \ref{tab:tab1}
	shows that $\N$ is a robust preconditioner for higher resolution.
	\\[1mm]
	\item Figures \ref{fig:fig3a_35}, \ref{fig:fig3b_35} give snapshots of the numerical solution along the iterations.
\end{itemize}
We conclude that in one-dimensional case \eqref{eq:hints}
exhibit very similar behavior to the hybrid method in \cite{zhang}
Yet, we use much less data to train Deeponet. We explain it by the fact that Deeponet is trained on functions with a fixed variance, and hence we must supply to the Deeponet values of the same order of magnitude as the ones used for training.
This is obtained using the constants $\varepsilon_i$ in \eqref{eq:hints}. 

\begin{figure}[!htb]
	\centering
	\begin{subfigure}[h]{0.5\textwidth}
		\includegraphics[scale=0.5]{figures/k_50/fig0.eps} 
		\caption{}
	\end{subfigure}
	\begin{subfigure}[h]{0.4\textwidth}
		\centering
		\includegraphics[scale=0.5]{figures/k_50/fig2.eps}
		\caption{}
	\end{subfigure}
	\caption{
		(A).  Neural network approximation vs exact solution. $f(x)=\sin(2\pi x)$ (left) and $f$ is Gaussian random field (right). $N=30, k=50 $. \\
		(B). Hints for \eqref{eq:helm} with $f=\sin(\pi x)+10\sin(3\pi x)+10\sin(5\pi x)$. $N=100,\theta=1, k=50 $
	}
	\label{fig:fig1}
\end{figure}


\begin{figure}[!htb]
	\centering
	\includegraphics[scale=0.9]{figures/k_35/fig3a.eps}
	\caption{Hints with $N=100,\theta=1, k=35 $}
	\label{fig:fig3a_35}
\end{figure}
\begin{figure}[!htb]
	\centering
	\includegraphics[scale=0.9]{figures/k_35/fig3b.eps}
	\caption{Hints for \eqref{eq:helm} with $f=\sin(\pi x)+10\sin(3\pi x)+10\sin(5\pi x)$. $N=100,\theta=1, k=35 $}
	\label{fig:fig3b_35}
\end{figure}
\newpage
\subsection{Training with corrupted Data}
\begin{table}[htb!]
	\centering
	\begin{tabular}{|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|}
		\hline
		$N$&$\varepsilon$& optimal $J$ &conv. rate&error& iterations	\\ [0.5ex]
		\hline
		$30$&1e-2& 5& 0.13&1.3e-14&242 \\[1mm]
		$60$&1e-2& 17& 0.043&6.3e-14&707 \\[1mm]
		$120$&1e-2& 34& 0.01&3.12e-13&2740 \\[1mm]
		$240$&1e-2& 93& 0.00262&1.5e-12&10,000\\[1mm]
		\hline
		\hline
		
		$30$&1e-14& 8& 0.16&1.3e-14&198 \\[1mm]
		$60$&1e-14& 13& 0.05&6.3e-14&593 \\[1mm]
		$120$&1e-13& 50& 0.01&3.12e-13&2160 \\[1mm]
		$240$&1e-13& 93& 0.003&7e-13&8548\\[1mm]
		\hline
	\end{tabular}
	\caption{Hints-GS for 1D-Helmholtz \eqref{eq:helm} with $k=50$ and $f=\sin(\pi x)+10\sin(3\pi x)+10\sin(5\pi x)$.
		$\varepsilon$ is given by 	\eqref{eq:epsilon}.
	}
	\label{tab:tab2}
\end{table}

A major drawback of Deeponet is the necessity of solving the equation many times.
This may take the sting out of its purpose.
Moreover, in practice, only approximated solutions can be obtained by direct methods for linear equations.
We are therefore interested in the following question:
Let $\hat{u}_i$ be approximated solutions to the system 
$Au_i=f_i$, such that
\begin{equation}\label{eq:epsilon}
	\frac{\|A\hat{u}_i-f\|_2}{\|f\|_2}<\varepsilon.
\end{equation}
We train the Deeponet with approximated solutions.
We are interested in the following question:\\
\begin{itemize}
	\item Does super-resolution behavior is maintained?
\end{itemize}
Table \ref{tab:tab2} shows that compromising the accuracy of the data set implies a slower convergence rate, yet, the number of iterations at the optimal $J$ differs by approximately a constant. Therefore, compromising the accuracy of the training set does not affect the super-resolution property.

In practice, we obtain $hatu_i$ using GMRES iterations up to a tolerance of $10-2$. As before, we train the system over $[0,1]$ with $N=30$ discretization points. For the sake of simplicity, we perform our experiments only for $k=50$. 


\subsection{Geometry transferability of Deeponet }
Let us   train Deeponet $\N_{\Gw}$ for solving \eqref{eq:helm}
in $\Gw=[0,1]^2$.
In the training process, we triangulate $\Gw$ with an averaged mesh diameter $h(\Gw)=0.1$.
The training data is generated as in 1D with Gaussian random fields defined on the interior nodes of the triangulation.
Then we would like to solve \eqref{eq:helm}  on a small perturbation of $\Gw$, which is an annular domain 
$\Gw\setminus B_{\varepsilon}$ where $B_{\varepsilon}$ is a rectangle with vertices
$$
(0.5,0.5), (0.5+\varepsilon, 0.5),
(0.5+\varepsilon, 0.5+\varepsilon), (0.5, 0.5+\varepsilon, )
$$
We would like to see whether a Deeponet trained for source domain $\Gw$, still provides robust preconditioner in \eqref{eq:hints} for iterative solver in a different perturbed domain.
Table \ref{tab:tab3} shows the convergence of the iterative method \eqref{eq:hints}  with $\N=\N_{\Gw}$ in the perturbed domain $\Gw\setminus B_{\varepsilon}$ in several resolutions  with $\varepsilon=0.1$.    $\N_{\Gw}$ has been trained on $\Gw$ and a resolution of $1/10$.
\begin{table}[htb!]
	\centering
	\begin{tabular}{|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|}
		\hline
		$h(\Gw_{\varepsilon})$&k&  $J$ &error& iterations	\\ [0.5ex]
		\hline
		$1/10$&40& 2& 3e-14&300 \\[1mm]
		$1/20$&40& 5&7e-14&1000 \\[1mm]
		$1/40$&40& 10&7e-14&4000 \\[1mm]
		\hline
	\end{tabular}
	\caption{Hints-GS for 2D-Helmholtz \eqref{eq:helm}
		in $\Gw\setminus B_{0.1}$ with $k=40$ and $f$ is a Gaussian random field defined on 
		$\Gw\setminus B_{0.1}$.}
	\label{tab:tab3}
\end{table}

As $\varepsilon$ increases, $\N$ does not provide a good preconditioner anymore, and the iterative method for $\Gw\setminus B_{\varepsilon}$ \eqref{eq:hints} did not converge.
